Public Transit for Special Events: Ridership Prediction and Train Optimization

Many special events, including sport games and concerts, often cause surges in demand and congestion for transit systems. Therefore, it is important for transit providers to understand their impact on disruptions, delays, and fare revenues. This paper proposes a suite of data-driven techniques that exploit Automated Fare Collection (AFC) data for evaluating, anticipating, and managing the performance of transit systems during recurring congestion peaks due to special events. This includes an extensive analysis of ridership of the two major stadiums in downtown Atlanta using rail data from the Metropolitan Atlanta Rapid Transit Authority (MARTA). The paper first highlights the ridership predictability at the aggregate level for each station on both event and non-event days. It then presents an unsupervised machine-learning model to cluster passengers and identify which train they are boarding. The model makes it possible to evaluate system performance in terms of fundamental metrics such as the passenger load per train and the wait times of riders. The paper also presents linear regression and random forest models for predicting ridership that are used in combination with historical throughput analysis to forecast demand. Finally, simulations are performed that showcase the potential improvements to wait times and demand matching by leveraging proposed techniques to optimize train frequencies based on forecasted demand.

==> sections/7_Recommendations.tex <==
\section{Recommendations}  

Due to their size and recurring nature, special events are an important consideration for transit operators as they often create disruptions, congestion, and overcrowding. Using the proposed techniques in this paper, transit agencies can understand the regularity to ridership for recurring events, such as sports games, and improve service quality and crowd management. 

\textbf{better demand matching}

To improve predictions for future events, transit agencies can reach out to the administration of event centers to try to get ticket sales for more accurate attendance estimates.

When comparing the pre-game and post-game ridership, the most used stations are the same. However, there is a major decrease in post-game ridership to the northernmost station on the Red Line, North Springs. Usually in the evenings, after 9:30, the red line does not run its whole route, so typically there is an extra transfer to make it all the way to North Springs. On game days, MARTA adjusts its schedule to provide full Red Line service to post-game riders. It is possible that improved marketing and advertisement might be able to recapture some of these riders, who might be unaware and using alternative means of transportation home, such as ridesharing. This could suggest the potential affects of an additional transfer on passenger behaviour. 

Currently, the majority of riders utilize the East and North directions
of trains post-game, so looking into potential directions to direct passengers to the stations West of the stadiums could be of interest. 
Given that stadium parking is often expensive and due to the large correlation previously noted between the amount of special-event ridership and the amount of parking available at each station, adjusting the amount of parking available at stations or the price of parking could be a interesting mechanism to help control passenger flow into stations. 
Additionally, partnerships with ride-sharing companies in a certain areas could be another way to attract more passengers to influence the demand for ridership. 

% Last but not least, MARTA can run their
% trains on a more optimal train schedule while ensuring that the safe
% capacity limit is followed. Reducing the amount of time between trains
% will help increase their service level at peak times while following
% recommended guidelines.

% In the case of MARTA, talking to officials at the Mercedes-Benz Stadium or State Farm Arena and asking for ticket sales figures of upcoming events would allow MARTA to get the attendance figures necessary for the model input in Section 6. 

% Transit agencies can plan in advance to reduce congestion and increase rider satisfaction: policies such as increased train frequency on certain corridors or custom routes during events due to popular origin/destination pairs can all help increase the efficiency of the system.

% Optimizing the line transfer process will also make more people
% interested in riding public transit as the inconvenience of
% transferring is removed. 





==> sections/oldSections/5_TrainScheduleEstimation_Clustering.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%]
% Section - Train Scheduling and Capacity Analysis
\section{Train Scheduling and Capacity Analysis}
\label{sec:TrainLevelClustering}
Beyond knowing simply the numbers of riders for events, it is also vital to gain an understanding of how those riders are being served. Some events lead to a overflow of demand for leaving the event locations, as a result, riders leaving the events can not get on their first trains. To alleviate the congestion level after the various events, train capacities are studied and an optimal schedule is proposed through a case study. The proposed framework of post-event ridership analysis can serve as a tool for rail managers schedule trains for a given size of event ridership. 



At the end of this section, a case study is performed for a soccer game. And a optimal train schedule is proposed for this event.  

\subsection{Train Schedule Estimation}
\label{sec:clustering method}

The analysis of event ridership on the train level is done through following steps. Detail of methods are described in section \ref{sec:clustering method}.
\begin{enumerate}
    \item Time Adjustment: To achieve a reasonable sample size for clustering, the start time and end time of each rider is adjusted to as if they travel along the same origin and destination. 
    \item Clustering: The event riders are grouped to their corresponding trains they took after the game based on their adjusted trip end times.
    \item Train Schedule estimation: The train schedule after the game is estimated from the clustering result. The train departure time at a station is approximated as the latest arrival time of the riders on that train at that station.
    \item Train Capacity Estimation: Simulations are performed for riders after the event with estimated train schedule using different train capacity, and train capacity which best matches the real data is selected.
\end{enumerate}

\subsubsection{Time Adjustment} 
\label{sec:Time Adjustment}
A time adjustment on the trips is applied before clustering to achieve better results with larger sample size. In this paper, the focus is on the origin-destination pairs of trips made on the same line (the East-West line). A baseline origin and destination pair is selected as target OD (eg. Dome/GWCC to East Lake). Passengers that may have different origins or destinations have their travel times adjusted as if they were traveling on the selected OD. In the case study, the start time and arrival time of post-event riders are adjusted as if they start from Dome/GWCC and arrive at East Lake. The result can be seen in the before and after images of \textbf{Figure \ref{fig:before-time-adjustment}} and \textbf{Figure \ref{fig:after-time-adjustment}}.
%For example, one scenario may be where the target OD is set to be Dome/GWCC to East Lake. If a passenger enters the Vine City station at 21:00 and arrives at Decatur station at 21:20, then this passenger's start time is shifted to 21:02 and end time is shifted to 21:17, as it normally takes 2 minutes to go from Vine City to Dome/GWCC (added to the start time) and 3 minutes to go from East Lake to Decatur (subtracted from the end time). Thus an estimation of time it takes for this person to travel from Dome/GWCC to East Lake can be generated. For this paper, start time is defined as the time when a rider taps their Breeze Card to enter a station, and end time is defined as the time when a rider taps their Breeze Card to leave a station. This process can be repeated for other riders to increase sample sizes for clustering. 

% %%%%%%%%%%%%% Time adjustment before & after %%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[th]
\centering
\includegraphics[width=1\linewidth]{figures/btimeadj.png}
\caption{Train passengers before time adjustment}
\label{fig:before-time-adjustment}
\end{figure}
\begin{figure}[th]
\centering
\includegraphics[width=1\linewidth]{figures/atimeadj.png}
\caption{Train passengers after time adjustment}
\label{fig:after-time-adjustment}
\end{figure}

\subsubsection{Hierarchical Density-Based Spatial Clustering of Applications with Noise (HDBSCAN)}
\label{sec:Clustering}
After adjusting start time and end time of the post-event trips, it can be observed from the data that riders that on the same train have similar end time of their trips. Therefore, riders are clustered on different trains based on their trip end time. HDBSCAN \cite{malzer2019hybrid} is the clustering algorithm is used on riders' arrival time at East Lake station. 

HDBSCAN is chosen because of its capable of clustering data in different densities and selecting clusters based on stability according to mutual reachability distance to build minimal spanning trees that then develop a cluster hierarchy.


The goal of this clustering is that each cluster of passengers were on the same unique train. This can be used to determine which train each passenger boarded, how long they boarded, and how many trains they waited. 

\subsubsection{Simulation}
An algorithm is proposed here which takes train capacity, train schedule, and riders' arrival time as input, and outputs clusters of passengers. 

This is used next to calculate the proportion-left-behind for each train, which is compared to simulation results to estimate the train capacity.

The goal of this simulation algorithm is to find the best train capacity that produces the proportion-left-behind for each train that matches the real congestion level after the event. 
Riders' arrival time comes from original data (i.e, data before time adjustment) after the event. 
With the passengers clustered on different trains for a specific OD pair, an estimated train departure time for the origin station is defined as the latest arrival time of that trains' passengers. 



\paragraph{Notation} 
\begin{itemize}
    \item $I$ denote the number of trains departing from the origin station
    \item $i$ be the index of the trains
    \item $S$ denote the set of all stations
    \item $s$ be the index of the stations
    % \item $s+k$ is the $k$-th next station along the trains' traveling direction.
    \item $T_i$ denotes the departure time of train $i$
    \item $C_{i,s}$ is the capacity of train $i$ at station $s$
\end{itemize}

\textbf{Algorithm \ref{left-behind calculation}} details how to perform a simulation of how passengers board the train using a FIFO queue and is used to calculate the proportion of passenger left behind for each train at each station.

, proportion of passengers that should get on their first train but get on the second train instead, on each train. 

\begin{algorithm}[h]
\SetAlgoLined
 $\text{demand left}_0$=0\;
 \For{i in 1:I}{
 New demand = Number of passengers arrive at station $s$ between $T_{i-1}$ and $T_{i}$\;
 $\text{Total demand}_i$ = $\text{demand left}_{i-1}$+ new demand \;
 $\text{demand left}_{i}$= $\text{max}(\text{total demand}_i-C_{i,s},0)$\;
 $C_{i,s+1}=\text{min}(0,C_{i,s}-\text{total demand}_i)$\;
 $\text{proportion left}_{i,s}=\frac{\text{demand left}_i}{\text{new demand}}$
 }
\caption{Simulation for a single station s}
\label{left-behind calculation}
\end{algorithm}


\subsection{Case Study Results}
\label{sec:train capacity}
\begin{comment}
    The game has an estimated ridership 10455.84.
\end{comment}
The Atlanta United game on September 22nd, 2018 is analyzed to estimate the maximum capacity of the train. In total, approximately 10813 people entered the Dome/GWCC and Vine City station after the game, which includes 3787 from Vine City and 7026 from Dome/GWCC. The event has no significant influence on the demand of other stations. 
%The two station signatures on September 22nd, 2018 are presented in \textbf{Figure \ref{fig:station signatures after 20180922}}.

To ensure a reasonable sample size, the people entering the Vine City and Dome/GWCC station after the game to Edgewood/Candler Park, East Lake, Decatur, Avondale, and Kensington are selected for analysis. Their trip start times and end times are shifted to their corresponding Dome/GWCC station to East Lake station time. These stations and their relative locations can be seen in  \textbf{Figure \ref{fig:MARTAmap}}. 

%\begin{figure*}[htp]
%\centering
%\begin{subfigure}{.5\textwidth}
%  \centering
%  \includegraphics[width=\linewidth]{figures/2018-9_22 VIne.png}
%  \caption{Vine City}
%  \label{fig:sub1}
%\end{subfigure}%
%\hfill
%\begin{subfigure}{.5\textwidth}
%  \centering
%  \includegraphics[width=\linewidth]{figures/2018-9_22 Dome.png}
%  \caption{Dome/GWCC}
%  \label{fig:sub2}
%\end{subfigure}
%\caption{September 22nd, 2018 Station Signatures}
%\label{fig:station signatures after 20180922}
%\end{figure*}

The most crowded start time period is investigated for passengers' shifted start times at Dome/GWCC station between 20:40:00 to 22:00:00. \textbf{Figure \ref{true dot plot 20180922}} shows these passengers' shifted start time and end time are in horizontal shaped clusters, and each horizontal shaped cluster corresponds passengers on the same train. 

\begin{figure}[th]
\centering
\includegraphics[width=1\linewidth]{figures/clustering Station Difference.png}
\caption{Start time V.S. End time for passengers entering Dome/GWCC station after ATL United game at Sep.22,2018}
\label{true dot plot 20180922}
\end{figure}

To assign the selected 2392 passengers at the target time interval on their corresponding trains, a HDBSCAN clustering is performed on the shifted end time of these passengers' trips with MinPts$= 50$. Initially, 12 clusters are detected by the HDBSCAN. The 21:45 and 21:49 trains are not separated by the HDBSCAN because the train at 21:45 has delay at some stations and, as a result, the shifted end time for the train at 21:45 are scattered. With the noise removed by the first run of HDBSCAN, a second HDBSCAN is run on the cluster with data from train at 21:45 and at 21:49. The two trains are separated on this subset of data. Eventually there are 13 clusters, which corresponds to 13 trains left Dome/GWCC after the game. The cluster results and the estimated train arrival time at Dome/GWCC station are presented on \textbf{Figure \ref{20180922 clustering result}}. The estimated train arrival times at Dome/GWCC station, which are plotted as dash lines on Figure \ref{20180922 clustering result}, are estimated as latest of the riders' arrival time in each train cluster since the clusters are generated by shifting start time and end time. In reality, passengers starting from Vine City have priority to board over passengers start from Dome Station.
%Two subplots are generated for the two subgroups of passengers, passengers from Vine City and passengers from Dome. 

%\textbf{Figure \ref{20180922 clustering result Vine}} and \textbf{Figure \ref{20180922 clustering result Dome}} shows the train clustering from \textbf{Figure \ref{20180922 clustering result}} broken down for Vine City passengers and Dome/GWCC passengers, respectively. 

\textbf{Figure \ref{Fig:start station}} shows the same riders as in \textbf{Figure \ref{20180922 clustering result}}. The colors in \textbf{Figure \ref{Fig:start station}} represents the start station of these post-event riders. From this figure, every train cluster has significant proportion of red dots, which means that all the 13 trains stopped at Dome/GWCC station. However, there are three trains that did not stop at Vine City station, which are trains at 21:09, 21:25, and, 21:45. These trains have no Vine City passengers and have a significant amount of Vine City passengers on the following trains. 

\textbf{Figure \ref{20180922 clustering result Dome}} is a subset of passengers in \textbf{Figure \ref{20180922 clustering result}}, only the passengers start their trips in Dome/GWCC are plotted in \textbf{Figure \ref{20180922 clustering result Dome}}. It is shown that during peak hours after the game, there are cases where riders cannot board their first train. For example, riders entering Dome/GWCC station between 21:09 and 21:12 got on the train at 21:12, 21:16, and 21:20 since the train arriving at Dome/GWCC at 21:09 was full. In this paper, we call these riders left-behind riders.

\begin{figure}[ht]
\centering
\includegraphics[width=1\linewidth]{figures/clustering results for ATL United Game new.png}
\caption{Train Clusters for passengers entering Dome/GWCC and Vine City station after ATL United game on September 22nd, 2018}
\label{20180922 clustering result}
\end{figure}

% %%%%%%%%% ----- Maybe add this back in when discuss some trains only go to one location ------ %%%%%%%%%%
% \begin{figure}[ht]
% \centering
% \includegraphics[width=1\linewidth]{figures/Start Station for each cluster.png}
% \caption{Start Stations for Riders after ATL United game on September 22nd, 2018}
% \label{Fig:start station}
% \end{figure}

% %%%%%%%%% ----- Probably leave out ------ %%%%%%%%%%
% \begin{figure}[ht]
% \centering
% \includegraphics[width=1\linewidth]{figures/Dome GWCC.png}
% \caption{Train Clusters for passengers entering Dome/GWCC station after ATL United game on September 22nd, 2018}
% \label{20180922 clustering result Dome}
% \end{figure}

Proportion of left-behind riders out of the total for each train is calculated for riders starting from Dome/GWCC station based on the train clusters. Rider arrival times are broken into 13 intervals. For example, riders who arrived between 20:52 and 21:00 are part of the demand for train at 21:00. The number of riders that travel Eastward from Dome/GWCC are calculated for each interval and they are listed as new demand. The proportion left-behind is the proportion of people did not get on their first train in each time interval. The proportion left-behind estimated at Dome/GWCC station is listed in \textbf{Table \ref{tab:simulation result}}


% Please add the following required packages to your document preamble:
\begin{table}[ht]
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{|c|c|c|}
\hline
Train Time & \begin{tabular}[c]{@{}c@{}c@{}} proportion left behind \\ estimated at Dome \\ from Cluster \end{tabular} & \begin{tabular}[c]{@{}c@{}} proportion left behind \\ 
simulated at Dome \\ 
% from Real data \\ 
(Maximum Capacity 707)\end{tabular} \\ 
% Train Time & 
% proportion left behind estimated at Dome from Cluster & 
% proportion left behind simulated at Dome from Real data (Maximum Capacity 707) \\
\hline
20:52 & 0.04 & 0.00 \\ \hline
21:00 & 0.11 & 0.18 \\ \hline
21:09 & 0.08 & 0.19 \\ \hline
21:12 & 0.60 & 0.70 \\ \hline
21:16 & 0.29 & 0.29 \\ \hline
21:20 & 0.16 & 0.00 \\ \hline
21:25 & 0.09 & 0.00 \\ \hline
21:29 & 0.37 & 0.31 \\ \hline
21:34 & 0.35 & 0.17 \\ \hline
21:39 & 0.12 & 0.00 \\ \hline
21:45 & 0.07 & 0.00 \\ \hline
21:49 & 0.00 & 0.00 \\ \hline
22:00 & 0.00 & 0.00 \\ \hline
\end{tabular}%
}
\caption{Proportions left behind in clusters and simulation}
\label{tab:simulation result}
\end{table}



The simulation \textbf{Algorithm \ref{left-behind calculation}} is used to calculate the proportion left behind testing with different train capacity at Dome/GWCC station. The algorithm takes the train schedule estimated from the clusters, arrival time of passengers, and a train capacity, and outputs a simulated proportion left-behind based on the input train capacity. The goal is to find a train capacity that minimizes the distance between the simulated proportion left-behind and the proportion left-behind in the train clusters at Dome/GWCC station. Here, the distance is measured by mean absolute error loss.  
 
\begin{figure}[ht]
\centering
\includegraphics[width=1\linewidth]{figures/Best Match train capacity New.png}
\caption{Minimization of MAE Loss function to find Maximum Capacity}
\label{loss function result}
\end{figure}
 
 As seen in \textbf{Figure \ref{loss function result}}, different numbers of riders per train are tested and the loss function is minimized. From the figure, maximum train capacity is 707, post-game. The simulated proportion left behind assuming the maximum train capacity is 707 is presented in \textbf{Table \ref{tab:simulation result}}. The real proportions are larger than the simulated proportion when the proportion-left-behind is small. This is due to the fact that in the simulation, it is assumed to be a perfect first-come-first-served rule. However, this is not the case in real situation. 
 
 The maximum capacity 707 is a lower bound estimation, because the double taps and people already on the trains (approximately a total of 35 people for the whole time period) are not counted here. These trains are 6-car trains post-game which have a stated maximum capacity of 576 people. From this analysis, however, one can see that the maximum capacity is often exceeded post-game. People often cram together in very close quarters as a result. It is also likely that being this far over stated capacity leads to increased risk of accident, injury, or illness. However, this is good evidence of peoples' tendency to ``pack it in" after sporting events.
 
 Under the assumption that people left behind from the previous train end up boarding on the next train before the new passengers for the next train do, the riders after the event wait a maximum of two trains, which corresponds to the case on \textbf{Figure \ref{20180922 clustering result}}. 

\subsubsection{Stability Analysis}

Since the train schedule is estimated as the time last person entering the Dome/GWCC station in each cluster, the true arrival time of the train could be later than the estimated time. Therefore, random noises are added to each train time and a maximum train capacity is calculated using Algorithm \ref{left-behind calculation}. 

\begin{figure}[h]
    \centering
    \includegraphics[width=0.8\linewidth]{figures/stability analysis New.png}
    \caption{Estimated Train Capacity after a random noise added}
    \label{stability}
\end{figure} 

Algorithm \ref{left-behind calculation} is run for 100 times. In each time, each train time is added by a random noise drawn from the positive side of a standard normal distribution (in minutes). A standard normal distribution is chosen because the trains are at least 2 minutes apart, and in reality, riders wait at most one train after the games. A train capacity estimation is calculated for each run. \textbf{Figure \ref{stability}} shows the results from 100 runs. The estimated train capacity has 1st quartile 699, 3rd quartile 720, mean 708 ,and median 706, which shows the algorithm is stable.



% \begin{comment}
% \subsection{Rail Clustering Comparison}
% Taking this clustering process, the next step is to compare clustering and estimated train schedules for different types of events. The clustering algorithm is run for a Hawks game on April 4th, 2018 with attendance of 16,696, a United game on June 2nd, 2018 with attendance of 45,140, and a Falcons game on September 23rd, 2018 with attendance 74,457.
% \begin{figure}[ht]
%     \centering
%     \includegraphics[width=\linewidth]{figures/hawks game cluster.png}
%     \caption{Atlanta Hawks Train Clustering}
%     \label{Hawks Train Cluster}
% \end{figure}
% \begin{figure}[ht]
%     \centering
%     \includegraphics[width=0.5\linewidth]{figures/Hawks Game Train Time table.png}
%     \caption{Hawks Estimated Train Arrivals}
%     \label{Hawks Train Arrivals}
% \end{figure}
% The clustering for the Hawks game is fairly straight forward. Everyone gets on their first choice train and train frequencies aren't adjusted for these events. There is minimal negative impact on the system. Trains arrive roughly every 20 minutes for these games.
% \begin{figure}[ht]
%     \centering
%     \includegraphics[width=\linewidth]{figures/ATL United Game cluster.png}
%     \caption{Atlanta United Train Clustering}
%     \label{ATLUTD Train Cluster}
% \end{figure}
% \begin{figure}[th]
%     \centering
%     \includegraphics[width=\linewidth]{figures/image (3).png}
%     \caption{Atlanta United Train Clustering by Destination}
%     \label{ATLUTD Train Cluster Dest}
% \end{figure}
% \begin{figure}[ht]
%     \centering
%     \includegraphics[width=0.3\linewidth]{figures/ATL United Traintime Upperdeck closed .png}
%     \caption{Atlanta United Estimated Train Arrivals}
%     \label{ATLUTD Train Arrivals}
% \end{figure}
% The Atlanta United games are a much more interesting case. The passengers can be clustered into 11 different trains. However, looking at train 4, all of the riders on that train are passengers on the green line. This is an interesting case that shows that both blue and green line trains are run post-game, despite the blue line covering all the green line stations anyway. This is a potential inefficiency that can be improved by only running blue lines. Trains seem to run in clumps as opposed to a consistent pattern. There is some congestion in the system, so not everyone is able to get on their first choice train.f
% \begin{figure}[ht]
%     \centering
%     \includegraphics[width=\linewidth]{figures/Falcons Game Cluster.png}
%     \caption{Atlanta Falcons Train Clustering by Destination}
%     \label{Falcons Train Cluster Dest}
% \end{figure}
% \begin{figure}[ht]
%     \centering
%     \includegraphics[width=0.3\linewidth]{figures/falcons traintime.png}
%     \caption{Atlanta Falcons Estimated Train Arrivals}
%     \label{Falcons Train Arrivals}
% \end{figure}
% Falcons games see some of the largest draws, and its ridership can be clustered into 14 different trains. Similar to the United games, not all passengers can get on their first choice train. However, there are no green line trains to be found here due to the clustering of blue line-only riders. Trains seem to run every 8 minutes except for a high traffic period when trains run every 5 minutes.

% This clustering analysis for different event types allows for the development of recommendations that can lead to changes in train frequency or line use for a more efficient way to quickly process all the riders.
% \end{comment}

\subsection{Optimal Train Schedule}
    An optimal train schedule is proposed for the Atlanta United game on September 22nd, 2018. \textbf{Figures \ref{20180922 clustering result Dome}} shows that the trains are crowded after the game at around 21:10 to 21:45. Some passengers even have to wait at the station for a second train. In this section, an ideal train schedule is proposed where every rider gets on their first train, and the trains are all operating at their safe capacity. 
    
    Assuming the train capacity is $n$ and using the adjusted time after the game as discussed in section \ref{sec:Time Adjustment}, the ith train arrival time at Dome/GWCC station is the shifted arrival time of the $i \times n$'th rider after the game. As a result, the first $n$ passengers would theoretically gets on the first train. Every $n$ consecutively arrived riders will get on the same train. The train schedule calculated in this method depends on which passenger is chosen as the first passenger after the game. But the train frequency is the important result to derive here.
    
    Assuming the train capacity is 576, which is the proposed safe capacity by MARTA, MARTA needs a train frequency of every 4 minutes to handle the peak hours from 21:00 to 21:40. If the train capacity is set to 707, which is the train capacity estimated from data from section \ref{sec:train capacity}, MARTA needs a train frequency of every 5 minutes to handle the peak hours from 21:00 to 21:40 after the game. The train schedules are presented in \textbf{Figure \ref{fig:optimal frequency}}.

\begin{comment}
    
\begin{table}[ht]
\centering
\resizebox{0.7\linewidth}{!}{%
\begin{tabular}{|c|c|c|}
\hline
\multicolumn{3}{|c|}{\textbf{Optimal Train Schedule After }} \\
\multicolumn{3}{|c|}{\textbf{ATL United Game on Sep 22, 2018}}
\\ \hline
\textbf{Actual} & \textbf{Capacity=576} & \textbf{Capacity =722} \\ \hline
& 20:52 &  \\ \hline
& 20:59 & 20:55 \\ \hline
& 21:03 & 21:01 \\ \hline
& 21:08 & 21:07 \\ \hline
& 21:12 & 21:12 \\ \hline
& 21:16 & 21:17 \\ \hline
& 21:20 & 21:22 \\ \hline
& 21:28 & 21:27 \\ \hline
& 21:32 & 21:32 \\ \hline
& 21:38 & 21:39 \\ \hline
& 21:45 & 21:50 \\ \hline
& 21:56 &  \\ \hline
\end{tabular}%
}
\caption{Actual rail schedule vs. optimal schedule for the 6 or 8 car trains.}
\label{tab:Optimal Train Schedules}
\end{table}
\end{comment}

\begin{figure}[ht]
        \centering
        \includegraphics[width=\linewidth]{figures/Optimal Train Schedule v2.png}
        \caption{Optimal Train Schedule After Atlanta United Game on Sep 22, 2018}
        \label{fig:optimal frequency}
\end{figure}

% \begin{comment}
%     \begin{figure}[ht]
%         \centering
%         \includegraphics[width=0.1\linewidth]{figures/optimal train schedule 576.png}
%         \caption{Optimal Train Schedule After Atlanta United Game on Sep 22, 2018 when train capacity is 576}
%         \label{fig:optimal 576}
%     \end{figure}
% \end{comment}   

    
    In comparing the optimal schedule and the true train schedule from Figure \ref{20180922 clustering result}, where 11 trains were used after the event, passengers arrived from 21:00 to 22:00. When using the proposed optimal schedule, 12 trains are needed from 21:00 to 22:00 to ensure the safe train capacity of 576. 10 trains are needed when assuming the train capacity is 707. Both the optimal train schedules outperform the actual train schedule in terms of reducing the number of trains riders have to wait before a successful boarding. In addition, the schedule in Figure \ref{fig:optimal frequency} with capacity 576 improves the safety of the train operation, while the schedule in Figure \ref{fig:optimal frequency} with capacity 707 reduces the operation cost after the game. 
    
    % \begin{comment}
    %     \begin{figure}[ht]
    %     \centering
    %     \includegraphics[width=0.1\linewidth]{figures/optimal 722.png} 
    %     \caption{Optimal Train Schedule After Atlanta United Game on Sep 22, 2018 when train capacity is 722}
    %     \label{fig:optimal 722}
    %     \end{figure}
    % \end{comment}
    
    
    % Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[H]
\centering
\resizebox{0.4\textwidth}{!}{%
\begin{tabular}{ccc}
\hline
Wait Time (Minutes) & Median  & 3rd Quantile \\ \hline
Original                  & 3.50                       & 5.72                      \\
Simulated (576 capacity) & 2.50                       & 3.73                      \\
Simulated (707 capacity) & 3.03                       & 4.55                     
\end{tabular}%
}
\caption{Wait Time Improvement}
\label{tab:Wait Time}
\end{table}

==> sections/oldSections/7_Predictions.tex <==
% \section{Ridership Prediction}
% % \subsection{Introduction}

% \subsection{Throughput Consistency}
% Given all this information about the system, the analyses in the previous sections be used in a predictive fashion for decision making. If MARTA can know the number of people entering a station at different times in advance, they can use the wait time metrics, capacity metrics, and origin/destination metrics to create optimal train schedules and routes that reduce waiting times and take passengers to their intended destinations quickly. In order to predict how people will enter a station, trip chains can be gathered into small bins for a set of similar events to determine and rider distribution. \textbf{Figure \ref{922utdthroughput}} shows the throughput of riders in five minute bins after an Atlanta United game where the upper deck of the stadium was opened.
% \begin{figure}[H]
%         \centering
%         \includegraphics[width=0.7\linewidth]{figures/922unitedthrougput3.png}
%         \caption{Post-game rider throughput at Dome/GWCC after Atlanta United game on September 22nd, 2018}
%         \label{922utdthroughput}
%         \end{figure}
% Similar figures can be generated from other similar games. Remarkably, the post-game throughput scenarios for Atlanta United games with the upper deck open shows strong consistency. When all the games are averaged and the rider numbers are converted to percentages, a sort of throughput signature can be generated. \textbf{Figure \ref{utdthroughputsig2}} depicts a consistent distribution that can be used to model the throughput after an Atlanta United game with the upper deck open. Using the consistent percentage throughput can be extrapolated based on the exact attendance of an Atlanta United game.
% \begin{figure}[H]
%         \centering
%         \includegraphics[width=0.7\linewidth]{figures/uts8.png}
%         \caption{Mean percentage rider throughput at Dome/GWCC after Atlanta United games with upper deck open}
%         \label{utdthroughputsig2}
%         \end{figure}
% \begin{figure}[H]
%       \centering
%         \includegraphics[width=0.7\linewidth]{figures/maxsdtpt.png}
%         \caption{Maximum rider throughput at Dome/GWCC after Atlanta United games with upper deck open}
%         \label{utdthroughputsig}
%         \end{figure}
% Looking at the upper bound figure, across all games in the sample, the maximum number of riders arriving in any bin is 615. Given that the train capacity is listed at 576, the combination of existing people waiting for a train, or people already on the train as it arrives will cause some passengers to either overcrowd or wait for the following train. If we look at the one standard deviation error bars, this can provide a good guidance of the worst-case situation MARTA needs to prepare for and can handle. If MARTA can manage passenger flow and train capacities in such a way that the maximum plus a standard deviation of passenger flow is managed, we know they can handle all situations less hectic than that.
% In addition to the overall distributions above, post-game, only 8\% of people take a train going west, while the rest of the riders wait for trains going east. Given these distributions, if a total number of riders post-game can be predicted, their stations entries, train waiting times, and destinations can all be predicted. The next part of the paper focuses on making those total ridership predictions.

% \subsection{Ridership Model Methods}
%     Given the knowledge of event locations, times, and attendance data, that can be combined with the ridership estimations for $r_a(t)$ from earlier in the paper to build a predictive model that can not only predict ridership, strictly speaking, but can also be used to gain a higher-fidelity analysis into rider behavior and system efficiency.
    
%     Multiple output types are calculated for the model to predict. The model can predict different types of ridership that are valuable in different scenarios. Those ridership types are listed below: 
%     \begin{enumerate}
%         \item Total ridership increment after a main sporting event near Dome/GWCC station and Vine City station. For Basketball games, equation $(1)$ is evaluated at the time interval 75 minutes to 195 minutes after the basketball game starts. For Football games, 30 to 420 minutes. And, for soccer, 60 to 300 minutes.
            
%         \item Ridership increment over the whole day when there are events near Dome/GWCC station and Vine City station. The number is calculated by evaluating equation $(1)$ over the whole day when there is an event. 
%     \end{enumerate}
%     \par The ridership for the events this paper builds models for is largely associated with the Dome/GWCC and Vine City stations. Using the bound estimation methods from earlier in the paper, events consistently cause large ridership changes from the baseline signature at these two stations. Riders do use other stations and occasionally spikes above average are found, but very minimally and inconsistently, leading to their removal from our ridership predictions. While other stations have activity and traffic as per usual, the lack of consistent deviation before or after events at the other stations leads to the assumption that the vast majority of riders alight at Dome/GWCC and Vine City. The ridership that the models aim to predict is a sum of the ridership values for the two stations. 
%     \par The three different model outputs described above will be referred to as Model (i) through Model (iii) where the number of i's refers to the output prediction type as listed above.
%     \par The models are focused on Atlanta Hawks games, Atlanta Falcons games, and Atlanta United games, as there are enough data points for those events to build strong models. These events are also among those that had the largest impact on ridership. The model is also useful for predicting the incidence of multiple events. While the model is more accurate predicting single large events, it also does a good job when taking into account a second event of equal or smaller size. Initially, there were two separate models for predicting single and multiple events, but a single model to predict multiple events actually performs just as well, if not better, on a single event subset.
        
%  \subsubsection{Attributes}
%  The attributes for each entry of the data are listed in \textbf{Table \ref{tab:attributes}}. For each model, the attributes input may vary. The Event 1 attendance in the model is based on the true attendance for sporting events compiled from the official league attendance records for each sports team. For single event instances, the solo sporting event comprises the Event 1 attributes, while the remaining attributes are set to NULL. For double event combinations where one event is a sporting event, the sporting event becomes Event 1 while the other event becomes Event 2. In instances where both events are sporting events, the sporting event with the later start time becomes Event 1. An example of a double event day is shown in \textbf{Figure \ref{Double Event Ex.}}. The later spike corresponds to Hawks v.s. Philadelphia 76ers game in State Farm Arena at 17:30. The earlier spike corresponds to MODEX 2018, an expo in Georgia World Congress Center, which starts at 10:00. The non-sporting events' riders leave the event at a much spread-out frame than the sporting events' riders. The non-sporting events also show a less intense spike than the sporting events. 
 
 
 
% \begin{table}[H]
% \centering
% \resizebox{\linewidth}{!}{%
% \begin{tabular}{|c|c|c|}
% \hline
%  & \textbf{Attributes} & \textbf{Type} \\ \hline
% \multirow{3}{*}{Event 1} & Category & Factor (Soccer/Football Game/Basketball - Hawks) \\ \cline{2-3} 
%  & Location & Factor(State Farm Arena/MBS/MBS\_Upper deck Open) \\ \cline{2-3} 
%  & Attendance & Numeric, True Attendance for Event 1 \\ \hline
%  & wpdiff2 & Home Team win percentage minus Away Team win percentage \\ \hline
%  & nadjsd & Margin of victory divided by standard deviation margin of victory for that league, negative if home team wins \\ \hline
% \multirow{3}{*}{Event 2} & Category 2 & Factor (15 Categories) \\ \cline{2-3} 
%  & Location 2 & Factor(GWCC/MBS/SFA/No  Location) \\ \cline{2-3} 
%  & Attendance 2 & Numeric (Attendance given in the SpecialEvents File) \\ \hline
% \multirow{4}{*}{} & time\_difference & time distance (in minutes) of the two events, 0 if there is no second event \\ \cline{2-3} 
%  & two\_event & Binary(True, if there is a second event) \\ \cline{2-3} 
%  & week & Binary(True, if the day is weekend) \\ \cline{2-3} 
%  & month & Factor(Month of the event) \\ \hline
% \end{tabular}%
% }
% \caption{Attributes}
% \label{tab:attributes}
% \end{table}
% \begin{figure}[H]
%         \centering
%         \includegraphics[width=0.7\linewidth]{figures/2018-4_10 two event.png}
%         \caption{Example of a double event day}
%         \label{Double Event Ex.}
%         \end{figure}
% \subsubsection{Machine Learning Models}
%     When predicting the ridership increment after main sporting event, there is a significant linear trend between the ridership increment and the attendance of the event as shown in \textbf{Figure \ref{LR model1}}.
%     \begin{figure}[H]
%         \centering
%         \includegraphics[width=\linewidth]{figures/LR model1.png}
%         \caption{Linear regression: y-axis is number of Riders after the event}
%         \label{LR model1}
%     \end{figure}
%         \begin{enumerate}
%             \item Linear Regression:
            
%             Linear regression fits the model in the form of 
%             \begin{equation}
%                 y=\mathbf{X}\hat{\beta}
%             \end{equation}
%             The coefficients of linear regression are estimated by method of least squares, which minimize the residual sum of squares:
%         \begin{equation}
%             RSS(\beta)=\sum^N_{i=1}(y_i-\beta_0-\sum_{j=1}^px_{ij}\beta_j)^2
%         \end{equation}



% \begin{table}[H]
% \centering
% \resizebox{\linewidth}{!}{%
% \begin{tabular}{c|c}
% \hline
% Models & Attributes Used in Reduced Linear Regression \\ \hline
% Model (i) & Attendance, Location2, Attendance 2 \\
% Model (ii) & Attendance,Location, Location2, Attendance 2 \\
% Model (iii) & Attendance,Location, Location2, Attendance 2 \\ \hline
% \end{tabular}%
% }
% \caption{Attributes used in Reduced Linear Regression }
% \label{linear regression attribtues}
% \end{table}


%         The attributes selected for each of the models are listed in \textbf{Table \ref{linear regression attribtues}}
%         \item Ridge Regression:
        
%         Ridge regression minimizes a penalized residual sum of squares:
%         \begin{equation}
%             \hat{\beta}^{ridge}=argmin_{\beta}\{\sum_{i=1}^N(y_i-\beta_0-\sum_{i=1}^px_{ij}\beta_j)^2+\lambda\sum_{j=1}^p\beta_j^2\}
%         \end{equation}
%         where $\lambda>0$, and $\lambda$ is chosen based on training data by cross-validation. And the ridge regression estimator is 
%         \begin{equation}
%             \hat{Y}=X_{n\times p}\hat{\beta}^{ridge}
%         \end{equation}
        
%         \item Regression Tree:
        
%         This model creates a set of nodes and branches where each particular set of input data selects a path down to an output node based on the criteria of the branches.
        
%         \item Random Forest Regression:
        
%         Random Forest Regression creates a set of regression trees and chooses the mean output value of all the trees to be the Random Forest Regression's output. Random Forest has two parameters, mtry, which is the number of variables randomly sampled at each split, and ntree, which is the number of trees to grow.
        
%         \item Support Vector Machine (SVM) Regression:
        
%         SVM has three parameters: gamma, epsilon, and cost. SVM regression sets decision boundary lines (epsilon) and then fits hyperplane to try and capture a maximal amount of points inside those decision boundaries. Using points within the decision boundaries gives a lower error rate and a better fit model. SVM regression models can also account for non-linearity. The kernel of an SVM model allows it to find higher dimensional hyperplanes without increasing the cost parameter.
        
%         %\item Bayesian Additive Regression Tree (BART)
        
%         \end{enumerate}
%         The machine learning is carried out using the R programming language. Specifically, the e1071 package is used for the SVM models, the package rpart is used for the regression trees, and the package randomForest is used for the random forest models.
        
%         The Random Forest and SVM models are tuned by grid search over a set of parameters and comparing the Root Mean Squared Error (RMSE). A variety of values are tried and the inputs that generate the lowest RMSE are used in the model. The results are shown in \textbf{Table \ref{tab:Parameters of Machine learning models} }. The SVM models all use the radial kernel.

% \begin{table}[H]
% \centering
% \resizebox{0.6\linewidth}{!}{%
% \begin{tabular}{|l|l|l|l|l|l|}
% \hline
%  & \multicolumn{2}{l|}{Random Forest} & \multicolumn{3}{l|}{SVM} \\ \hline
%  & Mtry & Number of trees & Gamma & Cost & Epsilon \\ \hline
% Model (i) & 5 & 1000 & 0.02631579 & 16 & 0 \\ \hline
% Model (ii) & 7 & 800 & 0.02631579 & 16 & 0.04 \\ \hline
% Model (iii) & 8 & 800 & 0.02631579 & 8 & 0.04 \\ \hline
% \end{tabular}%
% }
% \caption{Parameters of Machine Learning models }
% \label{tab:Parameters of Machine learning models}
% \end{table}

% \todo[inline]{“The results of the grid search are shown in Table 5”. What does that mean? What is the results? How is it computed and evaluated?}
%         \subsubsection{Performance Measurements}
%         This paper looks at the Mean Absolute Percentage Error (MAPE) and Mean Square Error (MSE) as the decision metrics. The goal is to build a model with \emph{at most} 20 percent MAPE. $\frac{1}{7}$ of the data set is reserved to be the testing set. A Monte Carlo Cross-Validation is run to ensure that the models perform consistently. The models are run 100 times and their testing errors are compared.
        
%         \begin{equation}
%             MAPE=\frac{1}{n}\sum_{i=1}^{n}|\frac{Y_i^{test}-f(x_i^{test})}{Y_i^{test}}|
%         \end{equation}
        
%         \begin{equation}
%             MSE=\frac{1}{n}\sum_{i=1}^{n}(Y_i^{test}-f(x_i^{test}))^2
%         \end{equation}
%         where n is the number of the samples in the test set and $f$ is the prediction function. 
%     \subsubsection{Monte Carlo Cross Validation}
%      Since the sample size is small, a Monte-Carlo Cross-Validation is followed. The computation is repeated 100 times for each method. In each iteration, the original data set is randomly split into testing data and training data. The Monte-Carlo Cross-Validation is seeded so that for each iteration, the testing set is consistent across model types. The performance for each methods, i.e. MSE and MAPE, is calculated for each test set. The average performance is calculated based on the following equations. N is defined as the number of repetitions, TE is the testing error, and n is the index.
%     \begin{equation}
%         \Bar{TE}=\frac{1}{N}\sum_{n=1}^{N}TE_n
%     \end{equation}
%     \begin{equation}
%         \hat{Var}(TE)=\frac{1}{N-1}\sum^{N}_{n=1}(TE_n-\Bar{TE})^2
%     \end{equation}
   

% \subsection{Ridership Prediction Results}

% After 200 runs of Monte Carlo Simulation,the average MSE and MAPE are calculated for all six model types. Below are the performances for each of the six model types in each category. The best performing model results are shown in \textbf{Table \ref{tab:Best Models}}. In addition to the primary model, two other models, Model 1 and Model 2, are introduced for the sake of comparison.

% \par    Model 1 is trained on single event days with attributes of the single event to compare the Primary Model's performance on single event days, while Model 2 is trained on all event days with attributes of the day's largest event to show the importance of secondary event information in prediction. The Primary Model is trained on all event days with attributes of all the day's events.

% \todo[inline]{Ridership not well-defined}    
% \begin{table}[H]
% \centering
% \resizebox{\linewidth}{!}{%
% \begin{tabular}{|c|c|c|c|}
% \hline
% \textbf{} & \textbf{Model 1:} & \textbf{Model 2:} & \textbf{Primary Model:} \\ \hline
% Inputs & \textbf{\begin{tabular}[c]{@{}c@{}}Single Event Days only \\ (78 days in 2018-2019)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}ALL event days \\ (136 days in 2018-2019)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}ALL event days \\ (136 days in 2018-2019)\end{tabular}} \\ \hline
% Attributes Included & \textbf{\begin{tabular}[c]{@{}c@{}}Category,Location,\\ Attendance,Week,Month\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Category,Location,Attendance,\\ Week,Month\end{tabular}} & \textbf{All Attributes listed in Table \ref{tab:attributes}} \\ \hline
% \textbf{\begin{tabular}[c]{@{}c@{}}i) Ridership Increment \\ After Main Sporting Event\end{tabular}} & RF: 11.73\% & LR:28.89\% & RF:16.55\% \\ \hline
% \textbf{\begin{tabular}[c]{@{}c@{}}ii) Ridership Increment \\ over whole day\end{tabular}} & RF:16.95\% & SVM:29.43\% & RF:16.98\% \\ \hline
% \textbf{iii) Ridership of the day} & RF: 10.68\% & SVM:21.71\% & SVM:11.89\% \\ \hline
% \end{tabular}%
% }
% \caption{Best Models }
% \label{tab:Best Models}
% \end{table}


% \begin{figure}[H]
%         \centering
%         \includegraphics[width=1\linewidth]{figures/Model 3ia.png}
%         \caption{\textbf{TO UPDATE} Primary Model (i) results}
%         \label{Model 3(i) results}
%         \end{figure}
% % \begin{figure}[H]
% %         \centering
% %         \includegraphics[width=1\linewidth]{figures/image (1).png}
% %         \caption{Primary Model (ii) results}
% %         \label{Model 3(ii) results}
% %         \end{figure}
% % \begin{figure}[H]
% %         \centering
% %         \includegraphics[width=1\linewidth]{figures/Model 3iiia.png}
% %         \caption{Primary Model (iii) results}
% %         \label{Model 3(iii) results}
% %         \end{figure}
% % \begin{figure}[H]
% %         \centering
% %         \includegraphics[width=1\linewidth]{figures/Model 1i.png}
% %         \caption{Model 1(i) results}
% %         \label{Model 1(i) results}
% %         \end{figure}
% % \begin{figure}[H]
% %         \centering
% %         \includegraphics[width=1\linewidth]{figures/Model 1ii.png}
% %         \caption{Model 1(ii) results}
% %         \label{Model 1(ii) results}
% %         \end{figure}
% % \begin{figure}[H]
% %         \centering
% %         \includegraphics[width=1\linewidth]{figures/Model 1iii.png}
% %         \caption{Model 1(iii) results}
% %         \label{Model 1(iii) results}
% %         \end{figure}
% % \begin{figure}[H]
% %         \centering
% %         \includegraphics[width=1\linewidth]{figures/Model 2i.png}
% %         \caption{Model 2(i) results}
% %         \label{Model 2(i) results}
% %         \end{figure}
% % \begin{figure}[H]
% %         \centering
% %         \includegraphics[width=1\linewidth]{figures/image (2).png}
% %         \caption{Model 2(ii) results}
% %         \label{Model 2(ii) results}
% %         \end{figure}
% % \begin{figure}[H]
% %         \centering
% %         \includegraphics[width=1\linewidth]{figures/Model 2iii.png}
% %         \caption{Model 2(iii) results}
% %         \label{Model 2(iii) results}
% %         \end{figure}

         
% \subsubsection{Analysis of different model types}
% \par Model 2 and the Primary Model in \textbf{Table \ref{tab:Best Models}} compare the effectiveness of models that take other events into consideration. In general, the effect of giving information (i.e. Category, Location, and Attendance) on a second event leads to 10 to 15 percent decrease in MAPE. This shows that even small events can have a quantifiable interactional impact on a bigger event and that it is important to take into account in transportation planning. Overall, the performance of the Primary Model over Model 2 also demonstrates the importance of second event information in gaining a better model result.
% \par On the whole, the Random Forest, SVM models tend to be perform the best in predicting the three scenarios. While Model 1 predicts ridership the best for single events, the Primary Model will be useful for multiple event predictions or in cases where a one-model-fits-all approach is needed. Model 1 and the Primary Model can help to serve in practical situations. Model 2, while a good benchmark for comparison in this paper, should not be used in real-life settings. 

% \par \textbf{Figures \ref{Model 3(i) results}, \ref{Model 3(ii) results}, and \ref{Model 3(iii) results}} show the Primary Models' prediction performance on single events days in addition to the overall result.We can compare these results with Model 1(i), Model 1(ii), and  Model 1(iii), which are designed to predict (i),(ii),and (iii) on for all single event days using only the single event days. Primary Model (i), Primary Model (ii), and Primary Model (iii) all show better performance on predicting single event days than Model 1(i), Model 1(ii), and Model 1(iii).This could because of the increased sample size of training data set. So Model 1 can be discarded, since the Primary Model has better performance on predicting single event days, as well as the ability to predict days with two events.

% \par Another advantage of these models is the ability to use their outputs to learn more in combination. Subtracting Primary Model (i)'s value from Primary Model (ii)'s value will yield a strong estimate for the number of riders to the target second smaller event. Previously, finding ridership estimates to a small event was difficult due to sample size restrictions or event size. In addition, Primary Model (iii) can also be used for a whole system understanding such as a trip chaining analysis or a simulation.

% \subsubsection{Important Attributes in the models}

% Random Forest is among the top two methods for predicting output types (i), (ii), and (iii). Random Forest also provides measurements of importance for the attributes, which is recorded as percent increase in the mean squared error (\%Inc MSE) for each attribute. The \% Inc MSE is calculated as following:
% \begin{enumerate}
%     \item Grow a random forest, each tree (t) in the random forest has a out-of-bag portion. Calculate the MSE for each tree (t) on their out-of-bag portion, call it $MSE_{t,0}$.
%     \item For each attribute j, permute the value of j in the out-of-bag portion in each tree. Calculate the MSE for each tree and call it $MSE_{t,j}$ 
%     \item For each attribute j, calculate the mean increase in accuracy $MInc_j=\frac{\sum_{\forall t}{MSE_{t,0}-MSE_{t,j}}}{\mbox{Number of Trees}}$ and the standard deviation of the difference $MSE_{t,0}-MSE_{t,j}$, call if $SD_j$
%     \item Return $\frac{MInc_j}{SD_j}$
% \end{enumerate}

% The \%Inc MSE are calculated for Primary Model (i), (ii), (iii). 
% \begin{figure}[H]
%     \centering
%     \includegraphics[width=0.5\linewidth]{figures/Model 3i importance.png}
%     \caption{percent increase in mean squared error of Primary Model (i)}
%      \label{model3i importance plot}
% \end{figure}
%     \textbf{Figure \ref{model3i importance plot}} shows that when predicting the ridership after the sporting event, the attendance of the event is the most important, followed by the location and category of the event. The Category of the second event on that day also has a sizeable impact on the prediction accuracy. That is due to the dataset having some 'big' events like concerts on the same day as a sporting event. Thus the second event has a fairly large impact on prediction accuracy. 
% \begin{figure}[H]
%     \centering
%     \includegraphics[width=0.5\linewidth]{figures/model2ii importance.png}
%     \caption{percent increase in mean squared error of Primary Model (ii)}
%     \label{model3ii importance plot}
% \end{figure}
% \begin{figure}[H]
%     \centering
%     \includegraphics[width=0.5\linewidth]{figures/Model3iii importance.png}
%     \caption{percent increase in mean squared error of Primary Model (iii)}
%     \label{model3iii importance plot}
% \end{figure}

% \textbf{Figure \ref{model3ii importance plot} and \ref{model3iii importance plot}} are very similar since they only differ by the addition of the 'mean ridership on weekday/weekend'. These figures show that when predicting the ridership for a specific day, attendance of both events are important, especially the sporting event, because the sporting events often have high attendance. 

% Overall, the attendance of the sporting event is the most important attribute for predicting ridership. An accurate estimation or calculation of the attendance can improve the accuracy of the prediction. In the research for this paper, two sets of attendance data for sporting events were used. The true attendance as described in the Attributes section is used in the analysis presented here. A less accurate estimation of attendance from the event dataset was also tried initially. When tried, the MAPE decreased by roughly 3\%. 


==> sections/oldSections/7_Predictions_new.tex <==
\section{Ridership Prediction}
\label{sec:ridership-prediction}
% \subsection{Introduction}


\subsection{Ridership Model Methods}
    Given the knowledge of event locations, times, and attendance data, that can be combined with the ridership estimations for $r_a(t)$ from earlier in the paper to build a predictive model that can not only predict ridership, strictly speaking, but can also be used to gain a higher-fidelity analysis into rider behavior and system efficiency.
    
    \par The ridership for the events this paper builds models for is largely associated with the Dome/GWCC and Vine City stations. Using the bound estimation methods from earlier in the paper, events consistently cause large ridership changes from the baseline signature at these two stations. Riders do use other stations and occasionally spikes above average are found, but very minimally and inconsistently, leading to their removal from our ridership predictions. While other stations have activity and traffic as per usual, the lack of consistent deviation before or after events at the other stations leads to the assumption that the vast majority of riders alight at Dome/GWCC and Vine City. The ridership that the models aim to predict is a sum of the ridership values for the two stations.
    
    Multiple output types are calculated for the model to predict. The model can predict different types of ridership that are valuable in different scenarios. Those ridership types are listed below: 
    \begin{enumerate}
        \item Total ridership increment after a main sporting event near Dome/GWCC station and Vine City station. For Basketball games, equation $(1)$ is evaluated at the time interval 75 minutes to 195 minutes after the basketball game starts. For Football games, 30 to 420 minutes. And, for soccer, 60 to 300 minutes.
            
        \item Ridership increment over the whole day when there are events near Dome/GWCC station and Vine City station. The number is calculated by evaluating equation $(1)$ over the whole day when there is an event. 
    \end{enumerate}
     
    \par The two different model outputs described above will be referred to as Model 1 and model 2.
    \par The models are focused on Atlanta Hawks games, Atlanta Falcons games, and Atlanta United games, as there are enough data points for those events to build strong models. These events are also among those that had the largest impact on ridership. The model is also useful for predicting the incidence of multiple events. While the model is more accurate predicting single large events, it also does a good job when taking into account a second event of equal or smaller size. Initially, there were two separate models for predicting single and multiple events, but a single model to predict multiple events actually performs just as well, if not better, on a single event subset.
    
    \subsubsection{Attributes}
 The attributes for each entry of the data are listed in \textbf{Table \ref{tab:attributes}}. For each model, the attributes input may vary. The Event 1 attendance in the model is based on the true attendance for sporting events compiled from the official league attendance records for each sports team. For single event instances, the solo sporting event comprises the Event 1 attributes, while the remaining attributes are set to NULL. For double event combinations where one event is a sporting event, the sporting event becomes Event 1 while the other event becomes Event 2. In instances where both events are sporting events, the sporting event with the later start time becomes Event 1. An example of a double event day is shown in \textbf{Figure \ref{Double Event Ex.}}. The later spike corresponds to Hawks v.s. Philadelphia 76ers game in State Farm Arena at 17:30. The earlier spike corresponds to MODEX 2018, an expo in Georgia World Congress Center, which starts at 10:00. The non-sporting events' riders leave the event at a much spread-out frame than the sporting events' riders. The non-sporting events also show a less intense spike than the sporting events. 
 
 
\begin{table}[h]
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{|c|c|p{3in}|}
\hline
 & \textbf{Attributes} & \textbf{Type} \\ \hline
\multirow{3}{*}{Event 1} & Category & Factor (Soccer/Football Game/Basketball - Hawks) \\ \cline{2-3} 
 & Location & Factor(State Farm Arena/MBS/MBS\_Upper deck Open) \\ \cline{2-3} 
 & Attendance & Numeric, True Attendance for Event 1 \\ \hline
 & wpdiff2 & Home Team win percentage minus Away Team win percentage \\ \hline
 & nadjsd & Margin of victory divided by standard deviation margin of victory for that league, negative if home team wins \\ \hline
\multirow{3}{*}{Event 2} & Category 2 & Factor (15 Categories) \\ \cline{2-3} 
 & Location 2 & Factor(GWCC/MBS/SFA/No  Location) \\ \cline{2-3} 
 & Attendance 2 & Numeric (Attendance given in the SpecialEvents File) \\ \hline
\multirow{4}{*}{} & time\_difference & time distance (in minutes) of the two events, 0 if there is no second event \\ \cline{2-3} 
 & two\_event & Binary(True, if there is a second event) \\ \cline{2-3} 
 & week & Binary(True, if the day is weekend) \\ \cline{2-3} 
 & month & Factor(Month of the event) \\ \hline
\end{tabular}
}
\caption{Attributes}
\label{tab:attributes}
\end{table}

\begin{table}[H]
\centering
\resizebox{0.5\linewidth}{!}{%
\begin{tabular}{|cc|}
\hline
\multicolumn{1}{|c|}{Primary Event} & Number of Days \\ \hline
Basketball -Hawks & 70 \\
Football Games & 28 \\
Soccer & 37 \\ \hline
\multicolumn{1}{|c|}{Day Type} & Number of Days \\ \hline
Single Event & 78 \\
Two Events & 57 \\ \hline
\end{tabular}%
}
\caption{Data Overview}
\label{tab:Data_overview}
\end{table}


\begin{figure}[h]
        \centering
        \includegraphics[width=0.7\linewidth]{figures/2018-4_10 two event.png}
        \caption{Example of a double event day}
        \label{Double Event Ex.}
\end{figure}

\subsubsection{Method}
There are 128 event days ranging from January 2018 to December 2019 that are used to fit the ridership prediction models. Because there is a small sample size of training data, a linear regression model is used to predict the mean response of ridership based on attributes provided. Then, all of the attributes are used to fit the residual of the linear regression.

Linear mean response model:
\begin{equation}
        \hat{\text{ridership}}=\hat{\beta_0}+\hat{\beta_1}\times \text{X} + \epsilon
\end{equation}
and random forests for predicting the residual of the linear regression model:
\begin{equation}
    \hat{\epsilon} = \frac{1}{B}\sum_{b=1}^B T_b(\textbf{x})
\end{equation}
where B is number of trees in the random forests model and x is the point that the model is trying to predict. The parameter $\beta$ is estimated by minimizing the residual sum of squares. B is estimated by fitting the model over different B values and find the best B that minimize the RMSE.
        
Leave-one-out cross validation to measure the accuracy of the prediction models. 
\subsection{Machine Learning Results}
\subsubsection{Model 1: Predicting Ridership increment after the main event}
From preliminary analysis, there exists a strong linear trend between the ridership increment and the attendance of the event. As shown in \textbf{Figure \ref{fig:ML model linear trend}}. Therefore a simple linear regression model with attendance of the main event as the single attribute can provide certain accuracy for our prediction. 

\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{figures/Model Result section Figures/Linear trend.png}
    \caption{Linear trend between attendance and ridership increment after the main event}
    \label{fig:ML model linear trend}
\end{figure}

Linear mean response model:
\begin{equation}
        \hat{\text{Ridership(x)}}=1169+0.1724\times \text{Attendance(x)} + \hat{\epsilon}
\end{equation}
The variance model predicting $\hat{\epsilon}$ is built using 800 trees with all attributes. \textbf{Table \ref{tab:result1}} shows the testing errors of three models types, simple linear regression model with attendance as the only attribute, our proposed linear regression with randoms forest model, and the random forests model with all attributes. The proposed simple linear regression with random forests model has the best performance in terms of MAE, MAPE, and RMSE. \textbf{Figure \ref{fig:residualFitted_LR}} and \textbf{Figure \ref{fig:residualFitted_LR+RF}} show the residual v.s. fitted plot of the linear model and the proposed linear model with variance model included. By fitting a separate variance model, the residuals decrease for most of the data points.

\begin{table}[h]
\centering
\resizebox{0.8\linewidth}{!}{%
\begin{tabular}{|c|c|c|c|}
\hline
        & \multicolumn{1}{c|}{\textbf{MAE}} &         \multicolumn{1}{c|}{\textbf{MAPE}} & \textbf{RMSE} \\ \hline
    \textbf{Simple LR} 
        & 498 
        & 0.1173    % 0.1172793 
        & 761.6     % 761.5958      
        \\ \hline
    \textbf{LR + RF}        
        & 494                               
        & 0.1157    % 0.1157123                         
        & 743.4   %  743.411
        \\ \hline
    \textbf{Random Forests} 
        & 577                               
        & 0.1405     % 0.1405140                
        & 844.9      % 844.9385
        \\ \hline
\end{tabular}%
}
\caption{prediction result for model 1}
\label{tab:result1}
\end{table}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.9\linewidth]{figures/Model Result section Figures/Simple Linear Model1.png}
    \caption{Residual v.s. Fitted plot for simple linear regression}
    \label{fig:residualFitted_LR}
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.9\linewidth]{figures/Model Result section Figures/LR+RF model1.png}
    \caption{Residual v.s. Fitted plot for simple linear regression and random forests}
    \label{fig:residualFitted_LR+RF}
 \end{figure}   
\subsubsection{Model 2: Predicting the ridership increment over the whole day}
The mean response model is built using the attributes Location, Attendance, Attendance2, week, and nadjsd. 

\textbf{Table \ref{tab:result2}} shows that the proposed combined model performs better than both linear regression model and random forests model in terms of MAE, MAPE, and RMSE. The residual v.s. fitted plots shown in \textbf{Figure \ref{fig:residualFitted_LR2} and \ref{fig:residualFitted_LR+RF2}} also show that adding a variance model helps reduce the error of prediction.

\begin{table}[h]
\centering
\resizebox{0.8\linewidth}{!}{%
\begin{tabular}{|c|c|c|c|}
\hline
                        & \multicolumn{1}{c|}{\textbf{MAE}} & \multicolumn{1}{c|}{\textbf{MAPE}} & \textbf{RMSE} \\ \hline
\textbf{Linear Regression}      
    & 635                               
    & 0.1586  % 0.1585618                          
    & 899.5 % 899.4691      
    \\ \hline
\textbf{LR + RF}        
    & 625                               
    & 0.1558  % 0.1558293                          
    & 877.0  % 877.0328       
    \\ \hline
\textbf{Random Forests} 
    & 731                               
    & 0.1797  % 0.1797470                          
    & 1007.6  % 1007.647  
    \\ \hline
\end{tabular}%
}
\caption{prediction result for model 2}
\label{tab:result2}
\end{table}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.9\linewidth]{figures/Model Result section Figures/Linear Regression 2.png}
    \caption{Residual v.s. Fitted plot for linear regression}
    \label{fig:residualFitted_LR2}
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.9\linewidth]{figures/Model Result section Figures/LR+RF2.png}
    \caption{Residual v.s. Fitted plot for linear regression and random forests}
    \label{fig:residualFitted_LR+RF2}
 \end{figure}   


==> sections/oldSections/Intro11_19.tex <==
% %---------------------------------------------
% %%%%%%%%%%%%%% ----- INTRO ---- %%%%%%%%%%%%

% \section{Introduction}
% \label{sec:intro}

% Many special events, including sports games, concerts, and festivals can often cause surges in demand and congestion for public transit systems. 
% Special events are an important consideration for transit providers in terms of the disruptions, delays, and fare revenue that they cause.
% % Special events can often be important sources of fare revenue for transit providers. 
% However, these surges in demand can also cause disruptions such as increased wait times due to congestion or delays for both event and non-event riders. 
% Due to their importance and nature of difficulty to plan for, special events are an important consideration for transit providers such as Metropolitan Atlanta Rapid Transit Authority (MARTA).

% % This has lead to much investment over the years both interms of research and data collection to help decision makers.
% % Large surveys can be expensive to conduct. AFC systems help the agencies have a better picture of both aggregate and individual level demand. 
% There has been a lot of investment over the years in studies to better understand patterns of public transit ridership in general and that related to special events. Initially, this was done mainly through surveying riders to build datasets \cite{KYTE1988345,doi:10.3141/2246-04}. 
% Automated Fare Collection (AFC) technologies have enabled more sophisticated analysis of transit ridership. This paper focuses on methods to use entry-exit AFC data to analyze current transit system performance and inform future planning decisions for special events.
% % Accurate predictions of event ridership and measures of impact on public transit systems can help operators better plan for these recurring events in order to provide better service and capture more ridership.

% % In order to analyze events, we start with baseline day in order to help us isolate the amount of demand that was specific to the special events. 
% % -- Want to see where riders are coming from / going to
% % -- One key question is what train are people getting on - only have gate times
% % -- One the important goals is to predict the number of riders for single or multiple events 
% % We also applied regression and machine learning techniques to predict the number of passengers for various events
% In Section \ref{sec:Ridership Analysis}, the ridership for non-event days is analyzed to create baseline signatures of entries and exits for each rail station on either weekdays or weekends. Ridership on event days is compared to baseline signatures to isolate event ridership. 
% In Section \ref{sec:od-analysis}, Trip chaining techniques are used to evaluate origin-destination (OD) pairs both at the aggregate level. 
% % One key method is applying HDBSCAN to infer the trains that individual passengers used on their trips.
% % Then, HDBSCAN is applied to identify which trains passengers boarded post game for analysis of average wait times and train loads. 
% These OD-pairs are also used in Section \ref{sec:TrainLevelClustering} to analyze train loads and wait times using HDBSCAN to perform train-level clustering. This is used to build regressions and machine learning models to predict post-game ridership.   

% % their post-game ridership demand and analyze its effect on the service level using entry-exit Automatic Fare Collection (AFC) data. This paper evaluates many machine learning methods for predicting post-game ridership of sports events and other nearby events using multiple years (2018-2019) of Breeze Card data for Atlanta, GA from the Metropolitan Atlanta Rapid Transit Authority (MARTA). 

% Overall, the focus of this paper is using these methods to answering the following key questions for MARTA:
% \begin{enumerate}[noitemsep]
%     \item How many passengers are arriving and departing from various locations?
%     \item What is the passenger load of the trains?
%     \item How long are individuals waiting for their trains?
%     \item How well can ridership be predicted for single or multiple nearby special events in the future?
% \end{enumerate}

% % In this paper, we focus on our methods to help answer key questions about special event ridership for MARTA to help them better analyze their performance and for future event scheduling. 
% Throughout this paper, the methods are then applied to multiple years of AFC rail data to provide analysis of the MARTA system in Atlanta, Georgia. The focus is on events located at the two stadiums downtown, Mercedes Benz arena (finished in 2017) and State Farm arena as well as the nearby convention centers, which hosts Atlanta United (first game 2017), the Falcons, and the Hawks. 
% % have multiple years of entry-exit AFC data that can be used to analyze the events. 
% % One key to note is that over the recent years some of the sports teams have moved locations to downtown, so the data is limited to the last few years. A lot of the events are in this area



% % The purpose in this paper is to understand the impact of riders on the system and how the system can better meet rider demands during events. To that end, analyses of rider origins and destinations are presented in this paper, as well as passenger clustering and simulation of train assignments. This paper also builds multiple models for different purposes and provides comparisons between the models. 

% %From the original analysis, the paper progresses to building machine learning models to predict ridership, as well as simulations to evaluated the effect of that ridership on system resources. User transit behaviors and rail ridership stickiness are also analyzed.

% % ----- END OF INTRO -------------
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> sections/oldSections/Intro1_20_21.tex <==
%---------------------------------------------
%%%%%%%%%%%%%% ----- INTRO ---- %%%%%%%%%%%%

\section{Introduction}
\label{sec:intro}

\textbf{Paragraph about:}\textit{ Public transit is very important for future. It has many potential societal and environmental benefits. Public transit helps ease congestion**. }


Special events, including sports games, concerts, and festivals, are an important consideration for transit providers due to their potential for the disruptions, delays, and fare revenue. The surges in demand and congestion from special events can have a negative impact on both special event and regular commuting ridership. Due to their impact and variance in nature, special events are an important consideration for transit providers.
% such as Metropolitan Atlanta Rapid Transit Authority (MARTA).

\textbf{Paragraph about:} \textit{Smart card technologies are giving us more info about happen. Still questions from transit planners about how to better predict and prepare for future events.}
Automated Fare Collection (AFC) technologies such as smart cards have enabled more sophisticated analysis of transit ridership. Initially, data collection and analysis focused on ridership surveys 
\cite{KYTE1988345, doi103141224604}. 
Studies in recent years have tried to better understand patterns of public transit ridership in general, as well as ridership related to special events.  Techniques and algorithms for helping to understanding past event ridership in order to better predict future event ridership and its impacts. 

Peak surges are after large events when everyone is leaving at the same time. 
Accurate predictions of event ridership and measures of impact on public transit systems can help operators better plan for these recurring events in order to provide better service and capture more ridership.

% The case study relies on a real data from the Metropolitan Atlanta Rapid Transit Authority (MARTA), 
Throughout this paper, the methods are then applied to multiple years (2018-2019?) of AFC rail data to provide analysis of the MARTA system in Atlanta, Georgia. The focus is on sporting events located at the two stadiums downtown, Mercedes Benz arena and State Farm arena, which have hosted the Atlanta Hawks, Falcons, and Atlanta United.
Present a case study for the city of Atlanta focused on the largest event centers
Stadium 1, stadium 2, convention center


% In order to analyze events, we start with baseline day in order to help us isolate the amount of demand that was specific to the special events. 
% -- Want to see where riders are coming from / going to
% -- One key question is what train are people getting on - only have gate times
% -- One the important goals is to predict the number of riders for single or multiple events 
% We also applied regression and machine learning techniques to predict the number of passengers for various events

This paper focuses on methods to use entry-exit AFC rail data at the station level for analysis of the transit system and prediction of event ridership in order to inform future planning decisions for special events. Some of the key questions presented to us by MARTA included: 
\begin{enumerate}[noitemsep]
    \item How many passengers are arriving and departing from various locations?
    \item What is the passenger load of the trains?
    \item How long are individuals waiting for their trains?
    \item How well can ridership be predicted for nearby special events in the future?
    \item Does the incidence of nearby smaller events have an impact on ridership to large special events?
\end{enumerate}

%-------- Contributions ------- 
% Contributions
% >1 - Detailed analysis of where people are coming from and the correlation with parking
% -- Analysis of the ridership shows some interesting correlation between parking, transfers, and lines
% >2 - Analysis of train
% From the data we are able 
% -- All the analysis of the trains is very interesting and novel
% -- from the breeze card data we can assess How congested are the trains and whether we can improve them for these events
% >3 - Consistency across the various events of how they are going to and from the trains (which allows us to do policies that are going to be applicable in general
% >4 -  Predict ridership pretty accurately 
% -- Using a simple prediction algorithm  (dont need something sophisticated to do a good job)

\paragraph{Contributions} 
This paper provides numerous technical and analytical contributions to help answer this questions. The introduction of station signatures showcases the regularity of ridership at the aggregate-level on non-event, baseline days. This allows for isolation of special event ridership. Through further analysis of event ridership origin-destination (OD) pairs highlights the strong correlation of ridership origins with parking locations. After the special event ridership has be
unsupervised learning techniques were used for train-level analysis to estimate train loads, wait-times, and capacity. These estimates were validated with simulation and compared to an proposed optimized schedule. 

are combined with simulation to generate optimal train schedules after special events. train-level analysis of congestion, wait-times, \& capacity. 
The final contribution is a relatively simple prediction algorithm/techniques that can be used to predict ridership pretty accurate, which is helpful for planners.
% % The analysis of this paper identifies the consistencies/regularity of human behavior at the aggregate level across the various events of how they are going to and from the trains, which allows for recommendations to be generalized in their applications for various types of special events. This paper includes a detailed analysis of where people are coming from and the correlation with parking. 

\paragraph{Outline} 
In Section \ref{sec:Ridership Analysis}, the ridership for non-event days is analyzed to create baseline signatures of entries and exits for each rail station on either weekdays or weekends. Ridership on event days is compared to baseline signatures to isolate event ridership.
In Section \ref{sec:od-analysis}, Trip chaining techniques are used to understand the locations of origin-destination (OD) pairs for special events at the aggregate level, as well as any patterns that may emerge from them. 
In Section \ref{sec:ridership-prediction}, regressions and machine learning models are used to predict post-game ridership, which along with analysis from previous section can be used to help inform transit planners. 
% One key method is applying HDBSCAN to infer the trains that individual passengers used on their trips.
In Section \ref{sec:TrainLevelClustering}, HDBSCAN is applied to identify which trains passengers boarded post game for analysis of average wait times and train loads. 
%These OD-pairs are also used in Section \ref{sec:TrainLevelClustering} to analyze train loads and wait times using HDBSCAN to perform train-level clustering. 


% their post-game ridership demand and analyze its effect on the service level using entry-exit Automatic Fare Collection (AFC) data. This paper evaluates many machine learning methods for predicting post-game ridership of sports events and other nearby events using multiple years (2018-2019) of Breeze Card data for Atlanta, GA from the Metropolitan Atlanta Rapid Transit Authority (MARTA). 
% The focus is on events located at the two stadiums downtown, Mercedes Benz arena (finished in 2017) and State Farm arena as well as the nearby convention centers, which hosts Atlanta United (first game 2017), the Falcons, and the Hawks. 
% have multiple years of entry-exit AFC data that can be used to analyze the events. 
% One key to note is that over the recent years some of the sports teams have moved locations to downtown, so the data is limited to the last few years. A lot of the events are in this area
% The purpose in this paper is to understand the impact of riders on the system and how the system can better meet rider demands during events. To that end, analyses of rider origins and destinations are presented in this paper, as well as passenger clustering and simulation of train assignments. This paper also builds multiple models for different purposes and provides comparisons between the models. 
% From the original analysis, the paper progresses to building machine learning models to predict ridership, as well as simulations to evaluated the effect of that ridership on system resources. User transit behaviors and rail ridership stickiness are also analyzed.

% ----- END OF INTRO -------------
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> sections/oldSections/otherAbstractNotes.tex <==


, which can be used to improve service level.

Using simulation and simple regression techniques, a representative ridership curve is predicted for 

proposed algorithm for simulation in combination with a prediction of special event ridership using linear regression and random forest prediction techniques, 

the potential improvements in train scheduling for special event ridership 

, prediction ridership for events using 


for post-game special event ridership. 
% simulate and optimize the train schedule to make it robust to help match supply and demand
Simulations are performed to validate the estimations of the train loads and passenger wait times. 
% applying regression and machine learning techniques to predict ridership of events



% Overall, the transit ridership for special events is shown to be relatively consistent to the extent that the analysis can be used as 

% The analysis of this paper identifies the consistencies of human behavior at the aggregate level across the various events of how, when and where special event ridership is using public transit system. which allows for recommendations to be generalized in their applications for various types of special events.
% Finally, this paper predicts ridership for events using regression and machine learning techniques. 
% Overall, the transit ridership for special events is shown to be relatively consistent to the extent that the analysis can be used as generalized insight for transit planners who are looking to better anticipate and manage demand for their services in the case of special events. 

% The special event ridership prediction along with the other analysis shows how the 
% With these predictions and throughput analysis, post-game train schedule recommendations can be made for future games. 
% The purpose of the analyses in the paper is to create a pipeline to predict post-game rider behavior at a high fidelity scale, from the ridership at a game, to their station entry, to their train boarding patterns, and to where they finally alight. 
% Recommendations
% The key contribution of this paper is providing techniques to help inform transit providers so they can 

% #######-------- Contributions --------#########
% Contributions
% >1 - Detailed analysis of where people are coming from and the correlation with parking
% -- Analysis of the ridership shows some interesting correlation between parking, transfers, and lines
% >2 - Analysis of train
% From the data we are able 
% -- All the analysis of the trains is very interesting and novel
% -- from the breeze card data we can assess How congested are the trains and whether we can improve them for these events
% >3 - Consistency across the various events of how they are going to and from the trains (which allows us to do policies that are going to be applicable in general
% >4 - Predict ridership pretty accurately 
% -- Using a simple prediction algorithm (dont need something sophisticated to do a good job)


% Recommendations are delivered as a result of the analyses on how MARTA may run their trains during events to improve key metrics.
% To that end, the Metropolitan Atlanta Rapid Transit Authority (MARTA) is interested in finding out how they can 
% From that analysis, an optimal train schedule is proposed to improve the train service efficiency and relieve the congestion after special events. 
% Measurements of impact and accurate predictions of event ridership on public transit systems can help operators better plan for these event-related surges in order to provide faster, safer service for larger amounts of riders. 

% The purpose of the analyses in the paper is to create a pipeline to predict post-game rider behavior at a high fidelity scale, from the ridership at a game, to their station entry, to their train boarding patterns, and to where they finally alight. Many special events, including sports games and concerts, can often cause surges in demand and congestion for public transit systems that can be hard to guess in advance. To that end, the Metropolitan Atlanta Rapid Transit Authority (MARTA) is interested in finding out how they can better anticipate and manage demand for their services in light of special events. Measurements of impact and accurate predictions of event ridership on public transit systems can help operators better plan for these event-related surges in order to provide faster, safer service for larger amounts of riders. After establishing baseline ridership in Atlanta for each rail station, this paper characterizes riders related to special events. The Atlanta case study includes analysis of the geographical distribution of event ridership and post-game congestion of the rail network using Automatic Fare Collection (AFC) data from MARTA. Simulations are performed to understand the service capabilities of the system, such as the proportion of riders that get left behind, train capacities, and rider wait times. From that analysis, an optimal train schedule is proposed to improve the train service efficiency and relieve the congestion after special events. Finally, machine learning models are established for predicting ridership counts for future events, which extends the method for quantifying ridership patterns for future events from the previous sections as well. Recommendations are delivered as a result of the analyses on how MARTA may run their trains during events to improve key metrics.


 %Additionally, optimization strategies are used to evaluate a maximum train capacity is estimated and simulation is performed after a game to establish optimal train scheduling.
